Improving robot navigation in crowded environments using intrinsic rewards

Autonomous navigation in crowded environments is an open problem with many applications, essential for the coexistence of robots and humans in the smart cities of the future. In recent years, deep reinforcement learning approaches have proven to outperform model-based algorithms. Nevertheless, even though the results provided are promising, the works are not able to take advantage of the capabilities that their models offer. They usually get trapped in local optima in the training process, that prevent them from learning the optimal policy. They are not able to visit and interact with every possible state appropriately, such as with the states near the goal or near the dynamic obstacles. In this work, we propose using intrinsic rewards to balance between exploration and exploitation and explore depending on the uncertainty of the states instead of on the time the agent has been trained, encouraging the agent to get more curious about unknown states. We explain the benefits of the approach and compare it with other exploration algorithms that may be used for crowd navigation. Many simulation experiments are performed modifying several algorithms of the state-of-the-art, showing that the use of intrinsic rewards makes the robot learn faster and reach higher rewards and success rates (fewer collisions) in shorter navigation times, outperforming the state-of-the-art.

==> sections/table-state-of-the-art.tex <==
\begin{table}[h]
    \centering
    \caption{Validation metrics of LSTM-RL, SARL and MP-RGL.}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{|c|c|c|c|c|}
    \hline
     \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{Exploration}} & \textbf{Average} & \textbf{Success} & \multirow{2}{*}{\textbf{Time}}
          \\ & & \textbf{return} & \textbf{rate} & \\
         \hline
         \multirow{2}{*}{\textbf{LSTM-RL}}
          & Original & 0.5841 & 0.903 & 11.683  \\
          & ICM & 0.5956 & 0.913 & 10.817  \\ \hline
        \multirow{2}{*}{\textbf{SARL}}
          & Original & 0.5660 & 0.890 & 11.674  \\
          & ICM & 0.5737 & 0.901 & 10.757  \\ \hline
          \multirow{2}{*}{\textbf{MP-RGL}}
          & Original & 0.6273 & 0.941 & 11.958  \\
          & ICM & 0.6437 & 0.956 & 11.274  \\ \hline
    \end{tabular}
    }

    \label{tab:table-state}
\end{table}
